Edge-Cuts and Rooted Spanning Trees

We give a closed form formula to determine the size of a k-respecting cut. Further, we show that for any k, the size of the k-respecting cut can be found only using the size of 2-respecting cuts.

==> sub_parts/add-sketch.tex <==
\begin{figure}
	\includegraphics[scale=0.45]{sub_parts/rough-sketch.png}	
	\caption{The figures represent the four cases dealt in the propositions. \newline In \CASE{1}, we have $x_i \perp_T x_j$ for all $i,j \in [k]$. This implies that $\gamma(\desc[T]{x_1},\desc[T]{x_2},\ldots,\desc[T]{x_k}) = 0$
		\newline In \CASE{2}, we have $\desc[T]{x_k} \supset \cdots \supset \desc[T]{x_2} \supset \desc[T]{x_1}$. This implies that $\gamma(\desc[T]{x_1},\desc[T]{x_2},\ldots,\desc[T]{x_k}) = \gamma(\desc[T]{x_k}, \desc[T]{x_1})$
		\newline  In \CASE{3}, we have $\desc[T]{x_k} \supset \desc[T]{x_a}\ \forall a < k, \exists i,j, x_i \perp_T x_j $. This implies that $\gamma(\desc[T]{x_1},\desc[T]{x_2},\ldots,\desc[T]{x_k}) = 0$
		\newline In \CASE{4}, $\exists Q' \subset Q$ such that 
		$\forall x \in Q'$, $\desc[T]{x_k} \supset \desc[T]x$ and 
		$\forall x \notin Q'$, $x_k \perp_T x$. This implies that $x_k$ can be left out. $\gamma(\desc[T]{x_1},\desc[T]{x_2},\ldots,\desc[T]{x_k}) = \gamma(\desc[T]{x_1},\desc[T]{x_2},\ldots,\desc[T]{x_{k-1}})$}
\end{figure}
